It Takes Two to Tango: Combining Visual and Textual Information for Detecting Duplicate Video-Based Bug Reports

When a bug manifests in a user-facing application, it is likely to be exposed through the graphical user interface (GUI). Given the importance of visual information to the process of identifying and understanding such bugs, users are increasingly making use of screenshots and screen-recordings as a means to report issues to developers. However, when such information is reported en masse, such as during crowd-sourced testing, managing these artifacts can be a time-consuming process. As the reporting of screen-recordings in particular becomes more popular, developers are likely to face challenges related to manually identifying videos that depict duplicate bugs. Due to their graphical nature, screen-recordings present challenges for automated analysis that preclude the use of current duplicate bug report detection techniques. To overcome these challenges and aid developers in this task, this paper presents Tango, a duplicate detection technique that operates purely on video-based bug reports by leveraging both visual and textual information. Tango combines tailored computer vision techniques, optical character recognition, and text retrieval. We evaluated multiple configurations of Tango in a comprehensive empirical evaluation on 4,860 duplicate detection tasks that involved a total of 180 screen-recordings from six Android apps. Additionally, we conducted a user study investigating the effort required for developers to manually detect duplicate video-based bug reports and compared this to the effort required to use Tango. The results reveal that Tango's optimal configuration is highly effective at detecting duplicate video-based bug reports, accurately ranking target duplicate videos in the top-2 returned results in 83% of the tasks. Additionally, our user study shows that, on average, Tango can reduce developer effort by over 60%, illustrating its practicality.

==> macro.tex <==
\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

% Merge citations into single brackets with commas
\usepackage[noadjust]{cite}
\renewcommand{\citepunct}{,\penalty\citepunctpenalty\,}
\renewcommand{\citedash}{--}% optionally

\newcommand\revised[1]{\textcolor{blue}{#1}}
\newcommand{\REF}{{\color{red} \textbf{[REFS]}}\xspace}
\newcommand\oscar[1]{\textcolor{olive}{\nb{OSCAR}{#1}}}
\newcommand\NATHAN[1]{\textcolor{blue}{\nb{NATHAN}{#1}}}
\newcommand\DENYS[1]{\textcolor{violet}{\nb{DENYS}{#1}}}
\newcommand\CARLOS[1]{\textcolor{orange}{\nb{CARLOS}{#1}}}
\newcommand\KEVIN[1]{\textcolor{violet}{\nb{KEVIN}{#1}}}
\newcommand{\num}{{\color{red} \textbf{XX}}\xspace}

\newcommand\NEW[1]{\nb{NEW}{#1}}
\newcommand{\tango}{{\textsc{Tango}}\xspace}
\newcommand{\tangos}{{\textsc{Tango}'s}\xspace}
\newcommand{\tangolong}{{\sc de\textbf{T}ecting duplic\textbf{A}te scree\textbf{N} recordin\textbf{G}s of s\textbf{O}ftware bugs}\xspace}


\newcommand{\tangot}{{\sc Tango$_{txt}$}\xspace}
\newcommand{\tangov}{{\sc Tango$_{vis}$}\xspace}
\newcommand{\tangoc}{{\sc Tango$_{comb}$}\xspace}


\newcommand{\bflcs}{B+f-LCS\xspace}
\newcommand{\bwlcs}{B+w-LCS\xspace}

==> tabs/all_apps_best.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c||c|c|c|c|c|c|c|}
    \hline
    \multicolumn{5}{|l||}{Configurations}                                 & \multicolumn{7}{c|}{Metrics}  \\
    \hline
    App & Model  & Approach  & FTK & VWs & mRR  & mAP & $\mu$ Rank & Rank $\sigma$ & HIT@1 & HIT@3  & HIT@5  \\
    \hline
    APOD & SIFT & w-lcs & 1 & 10k & 64.6\% & 51.1\% & 3.0 & 3.2 & 47.7\% & 78.5\% & 80.0\% \\
    APOD & SimCLR & bovw & 5 & 1k & 80.0\% & 66.8\% & 1.7 & 1.3 & 68.1\% & 91.5\% & 97.8\% \\
    APOD & OCR\&IR & all-text & 1 & N/A & 81.8\% & 74.2\% & 1.4 & 0.7 & 67.2\% & 98.0\% & 99.9\% \\
    \hline
    DROID & SIFT & w-lcs & 1 & 10k & 66.3\% & 55.0\% & 2.5 & 2.3 & 49.1\% & 80.1\% & 88.4\% \\
    DROID & SimCLR & bovw & 5 & 10k & 72.3\% & 61.4\% & 2.3 & 2.0 & 59.3\% & 78.1\% & 89.4\% \\
    DROID & OCR\&IR & uni-f & 5 & N/A & 72.4\% & 66.0\% & 2.0 & 1.5 & 55.9\% & 85.2\% & 95.1\% \\
    \hline
    GNU & SIFT & w-lcs & 1 & 10k & 66.1\% & 57.2\% & 2.2 & 1.6 & 47.4\% & 81.2\% & 94.2\% \\
    GNU & SimCLR & bovw & 5 & 5k & 82.9\% & 72.5\% & 1.5 & 1.0 & 71.5\% & 94.4\% & 99.9\% \\
    GNU & OCR\&IR & uni-w & 5 & N/A & 85.2\% & 78.8\% & 1.3 & 0.5 & 71.6\% & 99.8\% & 100.0\% \\
    \hline
    GROW & SIFT & bovw & 5 & 1k & 74.5\% & 67.3\% & 2.3 & 2.2 & 64.0\% & 81.1\% & 88.3\% \\
    GROW & SimCLR & bovw & 5 & 5k & 77.4\% & 75.1\% & 1.9 & 1.7 & 65.1\% & 87.9\% & 95.7\% \\
    GROW & OCR\&IR & all-text & 1 & N/A & 77.4\% & 70.8\% & 1.9 & 1.7 & 64.1\% & 90.7\% & 94.6\% \\
    \hline
    TIME & SIFT & w-lcs & 1 & 5k & 49.9\% & 40.9\% & 3.2 & 2.4 & 26.4\% & 68.3\% & 86.7\% \\
    TIME & SimCLR & bovw & 5 & 1k & 74.8\% & 67.6\% & 2.3 & 2.4 & 63.7\% & 80.9\% & 90.1\% \\
    TIME & OCR\&IR & all-text & 5 & N/A & 47.4\% & 37.7\% & 4.0 & 3.1 & 28.3\% & 57.0\% & 70.6\% \\
    \hline
    TOK & SIFT & w-lcs & 5 & 5k & 44.3\% & 35.9\% & 4.2 & 3.2 & 24.4\% & 52.0\% & 73.0\% \\
    TOK & SimCLR & bovw & 5 & 1k & 77.7\% & 69.3\% & 1.6 & 0.9 & 60.6\% & 96.4\% & 99.8\% \\
    TOK & OCR\&IR & all-text & 5 & N/A & 61.3\% & 53.3\% & 2.6 & 2.1 & 42.6\% & 77.0\% & 88.4\% \\
    \hline
    \hline
    ALL & SIFT & w-lcs & 1 & 10k & 56.9\% & 47.7\% & 3.1 & 2.6 & 37.4\% & 57.3\% & 70.7\% & 78.3\% & 83.0\% \\
    ALL & SimCLR & bovw & 5 & 1k & 75.3\% & 67.8\% & 1.9 & 1.7 & 61.6\% & 78.0\% & 86.7\% & 91.3\% & 95.0\% \\
    ALL & OCR\&IR & all-text & 5 & N/A & 69.8\% & 63.7\% & 2.3 & 2.1 & 54.1\% & 72.6\% & 82.6\% & 87.6% & 90.8\% \\
    \hline
    \end{tabular}
    \newline
    \caption{Top Configurations per model per app \NATHAN{TODO: Remove standard deviation, fix }}
    \label{tab:all_best}
\end{table*}

==> tabs/all_apps_best_combined.tex <==
% \begin{table*}[]
% \centering
% \caption{Top Configuration per combined model per app}
% \label{tab:all_best_combined_ocr}
% \begin{tabular}{c|c|ccc|ccccc}
% \hline
% \textbf{App}             & \textbf{W}                     & \textbf{mRR} & \textbf{mAP} & \textbf{μ Rank} & \textbf{H@1} & \textbf{H@2} & \textbf{H@3} & \textbf{H@4} & \textbf{H@5} \\ \hline
% APOD                     & 0.8 / 0.2                      & 84.4\%       & 75.8\%       & 1.4             & 73.1\%       & 87.9\%       & 98.5\%       & 99.9\%       & 100.0\%      \\ %\hline
% APOD                     & 1.0 / 0.0                      & 80.0\%       & 66.8\%       & 1.7             & 68.1\%       & 82.6\%       & 91.5\%       & 93.3\%       & 97.8\%       \\ %\hline
% APOD                     & 0.0 / 1.0                      & 80.8\%       & 75.3\%       & 1.5             & 65.7\%       & 88.6\%       & 98.3\%       & 99.1\%       & 100.0\%      \\ \hline
% DROID                    & 0.8 / 0.2                      & 70.6\%       & 66.7\%       & 2.2             & 55.9\%       & 71.0\%       & 80.7\%       & 89.3\%       & 93.6\%       \\ %\hline
% DROID                    & 1.0 / 0.0                      & 64.6\%       & 59.2\%       & 2.6             & 49.5\%       & 61.7\%       & 72.3\%       & 82.2\%       & 89.0\%       \\ %\hline
% DROID                    & 0.0 / 1.0                      & 67.9\%       & 64.7\%       & 2.3             & 52.0\%       & 69.8\%       & 78.4\%       & 86.9\%       & 91.6\%       \\ \hline
% GNU                      & 0.8 / 0.2                      & 89.5\%       & 84.7\%       & 1.3             & 81.6\%       & 94.2\%       & 96.8\%       & 99.0\%       & 99.6\%       \\ %\hline
% GNU                      & 1.0 / 0.0                      & 81.8\%       & 75.1\%       & 1.6             & 70.1\%       & 85.3\%       & 93.3\%       & 97.0\%       & 98.4\%       \\ %\hline
% GNU                      & 0.0 / 1.0                      & 84.5\%       & 82.3\%       & 1.4             & 72.2\%       & 92.0\%       & 96.9\%       & 99.1\%       & 99.9\%       \\ \hline
% GROW                     & 0.8 / 0.2                      & 81.7\%       & 75.4\%       & 1.7             & 71.4\%       & 82.5\%       & 92.8\%       & 95.6\%       & 96.4\%       \\ %\hline
% GROW                     & 1.0 / 0.0                      & 72.7\%       & 68.8\%       & 2.0             & 57.4\%       & 75.6\%       & 86.0\%       & 90.6\%       & 95.2\%       \\ %\hline
% GROW                     & 0.0 / 1.0                      & 76.8\%       & 69.0\%       & 1.9             & 63.6\%       & 80.1\%       & 87.7\%       & 92.6\%       & 94.4\%       \\ \hline
% TIME                     & 0.8 / 0.2                      & 59.6\%       & 51.7\%       & 2.8             & 40.2\%       & 58.8\%       & 74.7\%       & 84.6\%       & 89.9\%       \\ %\hline
% TIME                     & 1.0 / 0.0                      & 74.8\%       & 67.6\%       & 2.3             & 63.7\%       & 75.9\%       & 80.9\%       & 86.4\%       & 90.1\%       \\ %\hline
% TIME                     & 0.0 / 1.0                      & 47.4\%       & 37.7\%       & 4.0             & 28.3\%       & 44.4\%       & 57.0\%       & 64.0\%       & 70.6\%       \\ \hline
% TOK                      & 0.8 / 0.2                      & 69.8\%       & 60.8\%       & 2.0             & 50.9\%       & 76.9\%       & 85.3\%       & 92.1\%       & 96.0\%       \\ %\hline
% TOK                      & 1.0 / 0.0                      & 77.7\%       & 69.3\%       & 1.6             & 60.6\%       & 86.7\%       & 96.4\%       & 98.1\%       & 99.8\%       \\ %\hline
% TOK                      & 0.0 / 1.0                      & 61.3\%       & 53.3\%       & 2.6             & 42.6\%       & 60.7\%       & 77.0\%       & 84.1\%       & 88.4\%       \\ \hline \hline
% ALL & 0.8 / 0.2 & 75.9\%       & 69.2\%       & 1.9             & 62.2\%       & 78.5\%       & 88.1\%       & 93.4\%       & 95.9\%       \\ %\hline
% ALL & 1.0 / 0.0                      & 75.3\%       & 67.8\%       & 1.9             & 61.6\%       & 78.0\%       & 86.7\%       & 91.3\%       & 95.0\%       \\ %\hline
% ALL & 0.0 / 1.0                      & 69.8\%       & 63.7\%       & 2.3             & 54.1\%       & 72.6\%       & 82.6\%       & 87.6\%       & 90.8\%       \\ \hline
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Top combined configuration, weight 0.8 on visual information and 0.2 on textual information, per app and overall.}
\label{tab:all_best_combined_ocr}
\begin{tabular}{c|l|ccc|ccccc}
\textbf{App}           & \textbf{Info Type}                   & \textbf{mRR} & \textbf{mAP} & \textbf{μ Rank} & \textbf{H@1} & \textbf{H@2} & \textbf{H@3} & \textbf{H@4} & \textbf{H@5} \\ \hline
\multirow{3}{*}{APOD}  & \tango_{vis + txt} & 84.4\%       & 75.8\%       & 1.4             & 73.1\%       & 87.9\%       & 98.5\%       & 99.9\%       & 100.0\%      \\ \cline{2-10} 
                       & \tango_{vis}       & 80.0\%       & 66.8\%       & 1.7             & 68.1\%       & 82.6\%       & 91.5\%       & 93.3\%       & 97.8\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 80.8\%       & 75.3\%       & 1.5             & 65.7\%       & 88.6\%       & 98.3\%       & 99.1\%       & 100.0\%      \\ \hline
\multirow{3}{*}{DROID} & \tango_{vis + txt} & 70.6\%       & 66.7\%       & 2.2             & 55.9\%       & 71.0\%       & 80.7\%       & 89.3\%       & 93.6\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 64.6\%       & 59.2\%       & 2.6             & 49.5\%       & 61.7\%       & 72.3\%       & 82.2\%       & 89.0\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 67.9\%       & 64.7\%       & 2.3             & 52.0\%       & 69.8\%       & 78.4\%       & 86.9\%       & 91.6\%       \\ \hline
\multirow{3}{*}{GNU}   & \tango_{vis + txt} & 89.5\%       & 84.7\%       & 1.3             & 81.6\%       & 94.2\%       & 96.8\%       & 99.0\%       & 99.6\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 81.8\%       & 75.1\%       & 1.6             & 70.1\%       & 85.3\%       & 93.3\%       & 97.0\%       & 98.4\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 84.5\%       & 82.3\%       & 1.4             & 72.2\%       & 92.0\%       & 96.9\%       & 99.1\%       & 99.9\%       \\ \hline
\multirow{3}{*}{GROW}  & \tango_{vis + txt} & 81.7\%       & 75.4\%       & 1.7             & 71.4\%       & 82.5\%       & 92.8\%       & 95.6\%       & 96.4\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 72.7\%       & 68.8\%       & 2.0             & 57.4\%       & 75.6\%       & 86.0\%       & 90.6\%       & 95.2\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 76.8\%       & 69.0\%       & 1.9             & 63.6\%       & 80.1\%       & 87.7\%       & 92.6\%       & 94.4\%       \\ \hline
\multirow{3}{*}{TIME}  & \tango_{vis + txt} & 59.6\%       & 51.7\%       & 2.8             & 40.2\%       & 58.8\%       & 74.7\%       & 84.6\%       & 89.9\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 74.8\%       & 67.6\%       & 2.3             & 63.7\%       & 75.9\%       & 80.9\%       & 86.4\%       & 90.1\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 47.4\%       & 37.7\%       & 4.0             & 28.3\%       & 44.4\%       & 57.0\%       & 64.0\%       & 70.6\%       \\ \hline
\multirow{3}{*}{TOK}   & \tango_{vis + txt} & 69.8\%       & 60.8\%       & 2.0             & 50.9\%       & 76.9\%       & 85.3\%       & 92.1\%       & 96.0\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 77.7\%       & 69.3\%       & 1.6             & 60.6\%       & 86.7\%       & 96.4\%       & 98.1\%       & 99.8\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 61.3\%       & 53.3\%       & 2.6             & 42.6\%       & 60.7\%       & 77.0\%       & 84.1\%       & 88.4\%       \\ \hline \hline
\multirow{3}{*}{ALL}   & \tango_{vis + txt} & 75.9\%       & 69.2\%       & 1.9             & 62.2\%       & 78.5\%       & 88.1\%       & 93.4\%       & 95.9\%       \\ \cline{2-10} 
                       & \tango_{vis}       & 75.3\%       & 67.8\%       & 1.9             & 61.6\%       & 78.0\%       & 86.7\%       & 91.3\%       & 95.0\%       \\ \cline{2-10} 
                       & \tango_{txt}       & 69.8\%       & 63.7\%       & 2.3             & 54.1\%       & 72.6\%       & 82.6\%       & 87.6\%       & 90.8\%       \\ \hline
\end{tabular}
\end{table*}






% \begin{table*}[]
%     % 
%     % \centering
%     \hspace*{-1.7cm}
%     \centering
%     \begin{tabular}{|l|p{1.6cm}|p{1.2cm}|p{0.7cm}|p{0.8cm}|p{0.7cm}||c|c|c|c|c|c|c|c|c|}
%     %\hline
%     \multicolumn{6}{|l||}{Configurations}                                 & \multicolumn{9}{c|}{Metrics}  \\
%     %\hline
%     App & Model  & Approach  & FTK & VWs & W & mRR  & mAP & $\mu$ Rank & Rank $\sigma$ & H@1 & H@2 & H@3 & H@4 & H@5  \\
%     %\hline
%     % APOD & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.2 / 0.8 & 81.9\% & 74.5\% & 1.4 & 0.7 & 66.5\% & 92.5\% & 98.8\% & 99.9\% & 100.0\% \\
%     % %\hline
%     % APOD & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 67.6\% & 50.4\% & 2.8 & 3.0 & 52.8\% & 70.2\% & 78.3\% & 83.5\% & 86.2\% \\
%     % %\hline
%     APOD & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.8 / 0.2 & 84.4\% & 75.8\% & 1.4 & 0.7 & 73.1\% & 87.9\% & 98.5\% & 99.9\% & 100.0\% \\
%     %\hline
%     APOD & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 80.0\% & 66.8\% & 1.7 & 1.3 & 68.1\% & 82.6\% & 91.5\% & 93.3\% & 97.8\% \\
%     %\hline
%     APOD & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 80.8\% & 75.3\% & 1.5 & 0.8 & 65.7\% & 88.6\% & 98.3\% & 99.1\% & 100.0\% \\
%     %\hline
%     % DROID & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.8 / 0.2 & 78.4\% & 66.8\% & 1.8 & 1.6 & 66.9\% & 79.6\% & 87.8\% & 92.1\% & 95.9\% \\
%     % %\hline
%     % DROID & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 59.8\% & 53.0\% & 3.0 & 2.6 & 43.3\% & 57.8\% & 68.9\% & 76.2\% & 84.2\% \\
%     % %\hline
%     DROID & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.8 / 0.2 & 70.6\% & 66.7\% & 2.2 & 1.8 & 55.9\% & 71.0\% & 80.7\% & 89.3\% & 93.6\% \\
%     %\hline
%     DROID & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 64.6\% & 59.2\% & 2.6 & 2.1 & 49.5\% & 61.7\% & 72.3\% & 82.2\% & 89.0\% \\
%     %\hline
%     DROID & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 67.9\% & 64.7\% & 2.3 & 2.0 & 52.0\% & 69.8\% & 78.4\% & 86.9\% & 91.6\% \\
%     %\hline
%     % GNU & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.8 / 0.2 & 85.0\% & 81.4\% & 1.4 & 0.7 & 73.6\% & 90.5\% & 97.3\% & 99.6\% & 100.0\% \\
%     % %\hline
%     % GNU & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 56.5\% & 52.2\% & 2.6 & 1.7 & 33.8\% & 57.2\% & 75.3\% & 84.2\% & 91.4\% \\
%     % %\hline
%     GNU & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.8 / 0.2 & 89.5\% & 84.7\% & 1.3 & 0.7 & 81.6\% & 94.2\% & 96.8\% & 99.0\% & 99.6\% \\
%     %\hline
%     GNU & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 81.8\% & 75.1\% & 1.6 & 1.1 & 70.1\% & 85.3\% & 93.3\% & 97.0\% & 98.4\% \\
%     %\hline
%     GNU & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 84.5\% & 82.3\% & 1.4 & 0.8 & 72.2\% & 92.0\% & 96.9\% & 99.1\% & 99.9\% \\
%     %\hline
%     % GROW & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.8 / 0.2 & 82.2\% & 73.5\% & 1.5 & 0.8 & 69.8\% & 85.6\% & 96.9\% & 99.4\% & 99.9\% \\
%     % %\hline
%     % GROW & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 64.1\% & 56.1\% & 2.5 & 2.0 & 47.3\% & 63.8\% & 74.9\% & 84.0\% & 88.6\% \\
%     % %\hline
%     GROW & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.7 / 0.3 & 81.9\% & 74.8\% & 1.7 & 1.5 & 72.0\% & 82.6\% & 91.7\% & 95.2\% & 96.5\% \\
%     %\hline
%     GROW & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 72.7\% & 68.8\% & 2.0 & 1.7 & 57.4\% & 75.6\% & 86.0\% & 90.6\% & 95.2\% \\
%     %\hline
%     GROW & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 76.8\% & 69.0\% & 1.9 & 1.6 & 63.6\% & 80.1\% & 87.7\% & 92.6\% & 94.4\% \\
%     %\hline
%     % TIME & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.9 / 0.1 & 49.5\% & 39.7\% & 3.2 & 2.3 & 26.0\% & 46.8\% & 67.8\% & 79.0\% & 85.2\% \\
%     % %\hline
%     % TIME & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 39.0\% & 33.4\% & 4.0 & 2.6 & 14.1\% & 35.9\% & 52.7\% & 66.0\% & 73.5\% \\
%     % %\hline
%     TIME & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.9 / 0.1 & 63.2\% & 58.1\% & 2.6 & 2.3 & 43.1\% & 66.3\% & 82.1\% & 89.5\% & 92.1\% \\
%     %\hline
%     TIME & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 74.8\% & 67.6\% & 2.3 & 2.4 & 63.7\% & 75.9\% & 80.9\% & 86.4\% & 90.1\% \\
%     %\hline
%     TIME & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 47.4\% & 37.7\% & 4.0 & 3.1 & 28.3\% & 44.4\% & 57.0\% & 64.0\% & 70.6\% \\
%     %\hline
%     % TOK & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 0.1 / 0.9 & 58.4\% & 52.0\% & 2.8 & 2.2 & 38.9\% & 58.6\% & 72.7\% & 79.8\% & 84.9\% \\
%     % %\hline
%     % TOK & SIFT / OCR\&IR & w-lcs / all-text & 1 / 5 & 10k / N/A & 1.0 / 0.0 & 38.0\% & 31.2\% & 4.6 & 3.1 & 17.0\% & 31.1\% & 47.2\% & 59.8\% & 64.9\% \\
%     % %\hline
%     TOK & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.9 / 0.1 & 70.3\% & 63.0\% & 1.9 & 1.3 & 51.4\% & 76.2\% & 88.4\% & 94.3\% & 97.4\% \\
%     %\hline
%     TOK & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 77.7\% & 69.3\% & 1.6 & 0.9 & 60.6\% & 86.7\% & 96.4\% & 98.1\% & 99.8\% \\
%     %\hline
%     TOK & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 61.3\% & 53.3\% & 2.6 & 2.1 & 42.6\% & 60.7\% & 77.0\% & 84.1\% & 88.4\% \\
%     %\hline
%     %\hline
%     ALL & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.9 / 0.1 & 76.0\% & 70.0\% & 1.9 & 1.6 & 62.6\% & 78.6\% & 87.3\% & 92.6\% & 95.1\% \\
%     %\hline
%     ALL & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 1.0 / 0.0 & 75.3\% & 67.8\% & 1.9 & 1.7 & 61.6\% & 78.0\% & 86.7\% & 91.3\% & 95.0\% \\
%     %\hline
%     ALL & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & 0.0 / 1.0 & 69.8\% & 63.7\% & 2.3 & 2.1 & 54.1\% & 72.6\% & 82.6\% & 87.6\% & 90.8\% \\
%     % %\hline
%     % SPLIT & SimCLR / OCR\&IR & bovw / all-text & 5 / 5 & 1k / N/A & (0.8 / 0.2) / (1.0 / 0.0) & 79.8\% & 73.2\% & 1.7 & 1.5 & 67.7\% & 83.0\% & 91.0\% & 94.7\% & 96.6\% \\
%     %\hline
%     \end{tabular}
%     \newline
%     \caption{Top Configurations per combined model per app \NATHAN{Not sure if having this table be so close to the edges violates any format rules. May need to drop some of the Hits} \NATHAN{TODO: Remove standard deviation}}
%     \label{tab:all_best_combined_ocr}
% \end{table*}

==> tabs/apod.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{7}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & VWs & mRR  & mAP & $\mu$ Rank & Rank \sigma  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
     SIFT & w-lcs & 1 & 10,000      & 64.62\% & 51.14\% & 3.02 & 3.15  & 47.7\% & 78.5\% & 80.0\%   \\
     SIFT & bovw & 5 &  5,000              & 64.05\% & 53.42\% & 2.75 & 2.60  & 47.3\% & 75.9\% & 85.7\%   \\
     SIFT & bovw & 5 &  10,000             & 63.09\% & 52.88\% & 2.62 & 2.27  & 45.3\% & 76.7\% & 89.6\%   \\
     SIFT & w-lcs & 5 & 1,000       & 62.81\% & 52.09\% & 2.52 & 2.18  & 42.2\% & 79.6\% & 91.0\%   \\
     SIFT & w-lcs & 1 & 1,000       & 62.31\% & 47.51\% & 2.28 & 1.53  & 40.1\% & 83.2\% & 95.8\%   \\
     SIFT & w-lcs & 5 & 10,000      & 62.05\% & 52.99\% & 2.71 & 2.23  & 44.4\% & 73.5\% & 85.6\%   \\
     \hline
    SimCLR  & bovw  & 5  & 1,000               & 80.03\% & 66.77\% & 1.68 & 1.27  & 68.1\% & 91.5\% & 97.8\%    \\
    SimCLR  & bovw  & 5  & 5,000               & 76.27\% & 68.31\% & 2.14 & 2.27  & 64.9\% & 83.2\% & 91.2\%    \\
    SimCLR  & bovw  & 5  & 10,000              & 75.10\% & 69.22\% & 1.94 & 1.65  & 61.1\% & 88.5\% & 94.9\%    \\
    SimCLR  & bovw  & 1  & 5,000               & 68.68\% & 62.28\% & 2.59 & 2.64  & 54.2\% & 78.3\% & 87.8\%    \\
    SimCLR  & bovw  & 1  & 1,000               & 67.23\% & 58.64\% & 2.25 & 1.88  & 49.1\% & 83.3\% & 94.4\%    \\
    SimCLR  & bovw  & 1  & 10,000              & 66.75\% & 58.12\% & 2.26 & 1.90  & 47.0\% & 84.4\% & 92.6\%    \\
    \hline
    OCR\&IR & all-text & 1 & N/A              & 81.79\% & 74.18\% & 1.45 & 0.74  & 67.2\% & 98.0\% & 99.9\%    \\
    OCR\&IR & all-text & 5 & N/A              & 80.76\% & 75.32\% & 1.48 & 0.77  & 65.7\% & 98.3\% & 100.0\%   \\
    OCR\&IR & uni-f & 5 & N/A         & 76.52\% & 69.00\% & 1.67 & 0.99  & 60.5\% & 93.2\% & 99.6\%    \\
    OCR\&IR & uni-f & 1 & N/A         & 74.36\% & 67.73\% & 1.68 & 0.90  & 55.3\% & 95.1\% & 100.0\%   \\
    OCR\&IR & uni-w & 5 & N/A          & 73.21\% & 65.10\% & 1.80 & 1.13  & 55.4\% & 91.2\% & 99.0\%    \\
    OCR\&IR & uni-w & 1 & N/A          & 71.07\% & 64.25\% & 1.89 & 1.18  & 52.8\% & 90.2\% & 98.8\%    \\
    \hline
    \end{tabular}
    \newline
    \caption{APOD-SIFT: Keeping only top 6 results due to space contraints}
    \label{tab:apod_top}
\end{table*}

==> tabs/apod_m00.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
     SIFT & weighted lcs & 1 & 10,000      & 64.62\% & 51.14\% & 3.02 & 3.15 & 2.00 & 47.7\% & 78.5\% & 80.0\%   \\
     SIFT & bovw & 5 &  5,000              & 64.05\% & 53.42\% & 2.75 & 2.60 & 2.00 & 47.3\% & 75.9\% & 85.7\%   \\
     SIFT & bovw & 5 &  10,000             & 63.09\% & 52.88\% & 2.62 & 2.27 & 2.00 & 45.3\% & 76.7\% & 89.6\%   \\
     SIFT & weighted lcs & 5 & 1,000       & 62.81\% & 52.09\% & 2.52 & 2.18 & 2.00 & 42.2\% & 79.6\% & 91.0\%   \\
     SIFT & weighted lcs & 1 & 1,000       & 62.31\% & 47.51\% & 2.28 & 1.53 & 2.00 & 40.1\% & 83.2\% & 95.8\%   \\
     SIFT & weighted lcs & 5 & 10,000      & 62.05\% & 52.99\% & 2.71 & 2.23 & 2.00 & 44.4\% & 73.5\% & 85.6\%   \\
    \hline
    %  SIFT & 1000 & 5 & lcs                & 61.70\% & 54.33\% & 2.87 & 2.56 & 2.00 & 45.3\% & 69.1\% & 87.2\%   \\
    %  SIFT & 5000 & 1 & weighted lcs       & 61.55\% & 47.70\% & 2.96 & 2.80 & 2.00 & 43.5\% & 75.3\% & 83.5\%   \\
    %  SIFT & 5000 & 1 & bovw               & 61.31\% & 45.93\% & 3.09 & 2.97 & 2.00 & 45.3\% & 70.5\% & 84.2\%   \\
    %  SIFT & 5000 & 5 & weighted lcs       & 61.13\% & 53.65\% & 2.82 & 2.46 & 2.00 & 42.2\% & 74.2\% & 84.6\%   \\
    %  SIFT & 1000 & 5 & bovw               & 58.54\% & 51.57\% & 3.06 & 2.53 & 2.00 & 42.0\% & 64.6\% & 83.1\%   \\
    %  SIFT & 10000 & 1 & bovw              & 55.97\% & 43.02\% & 3.23 & 2.96 & 2.00 & 35.3\% & 69.6\% & 84.6\%   \\
    %  SIFT & 1000 & 1 & lcs                & 53.94\% & 41.73\% & 3.25 & 2.87 & 2.00 & 32.3\% & 69.0\% & 85.7\%   \\
    %  SIFT & 1000 & 1 & bovw               & 53.14\% & 42.79\% & 3.46 & 2.89 & 2.00 & 33.5\% & 64.7\% & 79.1\%   \\
    %  SIFT & 10000 & 5 & lcs               & 52.02\% & 45.94\% & 3.19 & 2.29 & 2.00 & 30.5\% & 60.4\% & 83.7\%   \\
    %  SIFT & 5000 & 5 & lcs                & 51.69\% & 46.16\% & 3.58 & 2.93 & 2.00 & 31.7\% & 61.9\% & 75.9\%   \\
    %  SIFT & 10000 & 1 & lcs               & 49.90\% & 40.59\% & 3.57 & 2.99 & 2.00 & 27.8\% & 63.2\% & 83.0\%   \\
    %  SIFT & 5000 & 1 & lcs                & 49.58\% & 40.43\% & 3.70 & 3.10 & 3.00 & 28.5\% & 64.7\% & 78.4\%   \\
    \end{tabular}
    \caption{APOD-SIFT: Keeping only top 6 results due to space contraints}
    \label{tab:apod m00}
\end{table*}

% \begin{table*}[]
%     \centering
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
%     \hline
%     Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    % \hline
%     \hline
%     \end{tabular}
%     \caption{Keeping only top 6 results due to space contraints}
%     \label{tab:apod m00}
% \end{table*}

==> tabs/apod_m01.tex <==
% \begin{tabular}{l|c|c|c|c|c|c|c|c}
% SimCLR  & 1000  & 5  & bovw               & 80.03\% & 66.77\% & 1.68 & 1.27 & 1.00 & 68.1\% & 91.5\% & 97.8\%    \\
% SimCLR  & 5000  & 5  & bovw               & 76.27\% & 68.31\% & 2.14 & 2.27 & 1.00 & 64.9\% & 83.2\% & 91.2\%    \\
% SimCLR  & 10000  & 5  & bovw              & 75.10\% & 69.22\% & 1.94 & 1.65 & 1.00 & 61.1\% & 88.5\% & 94.9\%    \\
% SimCLR  & 5000  & 1  & bovw               & 68.68\% & 62.28\% & 2.59 & 2.64 & 1.00 & 54.2\% & 78.3\% & 87.8\%    \\
% SimCLR  & 1000  & 1  & bovw               & 67.23\% & 58.64\% & 2.25 & 1.88 & 2.00 & 49.1\% & 83.3\% & 94.4\%    \\
% SimCLR  & 10000  & 1  & bovw              & 66.75\% & 58.12\% & 2.26 & 1.90 & 2.00 & 47.0\% & 84.4\% & 92.6\%    \\
% SimCLR  & 10000  & 5  & lcs               & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
% SimCLR  & 1000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
% SimCLR  & 5000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
% SimCLR  & 10000  & 1  & weighted_lcs      & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
% SimCLR  & 1000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
% SimCLR  & 5000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
% SimCLR  & 10000  & 5  & weighted_lcs      & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
% SimCLR  & 1000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
% SimCLR  & 5000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
% SimCLR  & 10000  & 1  & lcs               & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
% SimCLR  & 1000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
% SimCLR  & 5000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
% \end{tabular}

\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
    SimCLR  & bovw  & 5  & 1,000               & 80.03\% & 66.77\% & 1.68 & 1.27 & 1.00 & 68.1\% & 91.5\% & 97.8\%    \\
    SimCLR  & bovw  & 5  & 5,000               & 76.27\% & 68.31\% & 2.14 & 2.27 & 1.00 & 64.9\% & 83.2\% & 91.2\%    \\
    SimCLR  & bovw  & 5  & 10,000              & 75.10\% & 69.22\% & 1.94 & 1.65 & 1.00 & 61.1\% & 88.5\% & 94.9\%    \\
    SimCLR  & bovw  & 1  & 5,000               & 68.68\% & 62.28\% & 2.59 & 2.64 & 1.00 & 54.2\% & 78.3\% & 87.8\%    \\
    SimCLR  & bovw  & 1  & 1,000               & 67.23\% & 58.64\% & 2.25 & 1.88 & 2.00 & 49.1\% & 83.3\% & 94.4\%    \\
    SimCLR  & bovw  & 1  & 10,000              & 66.75\% & 58.12\% & 2.26 & 1.90 & 2.00 & 47.0\% & 84.4\% & 92.6\%    \\
    % SimCLR  & 10000  & 5  & lcs               & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
    % SimCLR  & 1000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
    % SimCLR  & 5000  & 5  & lcs                & 60.65\% & 55.08\% & 2.67 & 2.28 & 2.00 & 40.5\% & 79.3\% & 89.4\%    \\
    % SimCLR  & 10000  & 1  & weighted_lcs      & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
    % SimCLR  & 1000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
    % SimCLR  & 5000  & 1  & weighted_lcs       & 59.07\% & 46.59\% & 3.13 & 3.03 & 2.00 & 38.8\% & 77.7\% & 82.2\%    \\
    % SimCLR  & 10000  & 5  & weighted_lcs      & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
    % SimCLR  & 1000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
    % SimCLR  & 5000  & 5  & weighted_lcs       & 55.01\% & 44.85\% & 3.27 & 2.72 & 2.00 & 35.7\% & 65.2\% & 83.7\%    \\
    % SimCLR  & 10000  & 1  & lcs               & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
    % SimCLR  & 1000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
    % SimCLR  & 5000  & 1  & lcs                & 52.85\% & 44.69\% & 3.19 & 2.41 & 2.00 & 32.1\% & 64.8\% & 84.2\%    \\
    \hline
    \end{tabular}
    \caption{APOD-SimCLR: Keeping only top 6 results due to space contraints}
    \label{tab:apod_m01}
\end{table*}


==> tabs/apod_ocr_ir.tex <==
% \begin{tabular}{l|c|c|c|c|c|c|c|c}
%  OCR \& IR & 1 & all text              & 81.79\% & 74.18\% & 1.45 & 0.74 & 1.00 & 67.2\% & 98.0\% & 99.9\%    \\
%  OCR \& IR & 5 & all text              & 80.76\% & 75.32\% & 1.48 & 0.77 & 1.00 & 65.7\% & 98.3\% & 100.0\%   \\
%  OCR \& IR & 5 & unique frames         & 76.52\% & 69.00\% & 1.67 & 0.99 & 1.00 & 60.5\% & 93.2\% & 99.6\%    \\
%  OCR \& IR & 1 & unique frames         & 74.36\% & 67.73\% & 1.68 & 0.90 & 1.00 & 55.3\% & 95.1\% & 100.0\%   \\
%  OCR \& IR & 5 & unique words          & 73.21\% & 65.10\% & 1.80 & 1.13 & 1.00 & 55.4\% & 91.2\% & 99.0\%    \\
%  OCR \& IR & 1 & unique words          & 71.07\% & 64.25\% & 1.89 & 1.18 & 1.00 & 52.8\% & 90.2\% & 98.8\%    \\
% \end{tabular}

\begin{table*}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Configurations}                           & \multicolumn{8}{c|}{Metrics}                                                                \\
    \hline
    Model  & Approach  & FTK & \# of VWs & $\mu$ Rank & Median Rank & Rank \sigma & mRR  & mAP  & HIT@1  & HIT@3  & HIT@5  \\
    \hline
    OCR \& IR & all text & 1 & N/A              & 81.79\% & 74.18\% & 1.45 & 0.74 & 1.00 & 67.2\% & 98.0\% & 99.9\%    \\
    OCR \& IR & all text & 5 & N/A              & 80.76\% & 75.32\% & 1.48 & 0.77 & 1.00 & 65.7\% & 98.3\% & 100.0\%   \\
    OCR \& IR & unique frames & 5 & N/A         & 76.52\% & 69.00\% & 1.67 & 0.99 & 1.00 & 60.5\% & 93.2\% & 99.6\%    \\
    OCR \& IR & unique frames & 1 & N/A         & 74.36\% & 67.73\% & 1.68 & 0.90 & 1.00 & 55.3\% & 95.1\% & 100.0\%   \\
    OCR \& IR & unique words & 5 & N/A          & 73.21\% & 65.10\% & 1.80 & 1.13 & 1.00 & 55.4\% & 91.2\% & 99.0\%    \\
    OCR \& IR & unique words & 1 & N/A          & 71.07\% & 64.25\% & 1.89 & 1.18 & 1.00 & 52.8\% & 90.2\% & 98.8\%    \\
    \hline
    \end{tabular}
    \caption{APOD OCR & IR: Keeping only top 6 results due to space contraints}
    \label{tab:apod_ocr_ir}
\end{table*}

==> tabs/overall_best.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|l|}{Configurations}                                 & \multicolumn{9}{c|}{Metrics}  \\
    \hline
    Model  & Approach  & FTK & VWs & mRR  & mAP & $\mu$ Rank & Rank $\sigma$ & H@1 & H@2 & H@3 & H@4 & H@5  \\
    \hline
    SIFT & w-lcs & 1 & 10k & 60.7\% & 51.7\% & 2.7 & 2.2 & 41.1\% & 63.1\% & 76.1\% & 81.7\% & 86.5\% \\
    SimCLR & bovw & 5 & 1k & 77.6\% & 70.6\% & 1.8 & 1.4 & 64.3\% & 81.1\% & 89.8\% & 93.7\% & 96.7\% \\
    OCR\&IR & all-text & 1 & N/A & 73.9\% & 68.0\% & 2.0 & 1.8 & 59.3\% & 77.8\% & 85.7\% & 91.3\% & 93.0\% \\
    \hline
    \end{tabular}
    \newline
    \caption{Top Configurations per model across all apps}
    \label{tab:all_best}
\end{table*}

==> tabs/setting2.tex <==
\begin{table}[]
\centering
\small
\caption{Examples of duplicate detection tasks for an app. B$x$-P$y$ represents a bug report from participant $y$ for bug $x$.
% \NATHAN{How does this look for explaining setting 2?}
% \oscar{I like it, but we should simplify it, make it clear, and ideally make it fit in one column.}
} 
\label{tab:setting2}
\setlength\tabcolsep{5pt} 
\begin{tabular}{c|cccccc}

\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}(Task \#)\\ Query\end{tabular}}} & \multicolumn{6}{c}{\textbf{Corpus}}                                                                                                                                                                                                                                               \\ \cline{2-7} 
                                & \multicolumn{4}{c|}{\textbf{Duplicate Groups}}                                                                                & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Non\\ Duplicates\end{tabular}}}} \\ \cline{2-5}
                                & \multicolumn{2}{c|}{\textbf{Same Bug}} & \multicolumn{2}{c|}{\textbf{Different Bug}} & \multicolumn{2}{c}{}                                                                                   \\ \bottomrule
(1) B1-P1                          & B1-P2                       & \multicolumn{1}{l|}{B1-P3}                      & B2-P1                           & \multicolumn{1}{c|}{...}                           & B3-P1                                               & ...                                              \\
(2) B1-P1                          & B1-P2                       & \multicolumn{1}{l|}{B1-P3}                      & B2-P1                           & \multicolumn{1}{c|}{...}                           & B3-P2                                               & ...                                              \\
(3) B1-P1                          & B1-P2                       & \multicolumn{1}{l|}{B1-P3}                      & B2-P1                           & \multicolumn{1}{c|}{...}                           & B3-P3                                               & ...                                              \\
$\vdots$                             & $\vdots$                             & \multicolumn{1}{c|}{$\vdots$}                            & \vdots                                 & \multicolumn{1}{c|}{$\vdots$}                              & $\vdots$                                                     & $\ddots$                                                 \\ 

%(810) B10-P1                          & B10-P2                       & \multicolumn{1}{l|}{B10-P3}                      & B1-P3                           & \multicolumn{1}{c|}{...}                           & B2-P3                                               & ...                                              \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table*}[]
% \centering
% \caption{Duplication task layout. B\#-P\# represents a bug report of bug \# from participant \#. \NATHAN{How does this look for explaining setting 2?}
% \oscar{I like it, but we should simplify it, make it clear, and ideally make it fit in one column.}
% } 
% \label{tab:setting2}
% \begin{tabular}{c|ccccccccc}
% \toprule
% \multirow{3}{*}{\textbf{Query}} & \multicolumn{9}{c}{\textbf{Corpus}}                                                                                                                   \\ \cline{2-10} 
%                                 & \multicolumn{5}{c|}{\textbf{Duplicate Groups}}                                         & \multicolumn{4}{c}{\multirow{2}{*}{\textbf{Non-Duplicates}}} \\ \cline{2-6}
%                                 & \multicolumn{2}{c|}{\textbf{Same Bug}} & \multicolumn{3}{c|}{\textbf{Different Bug}}   & \multicolumn{4}{c}{}                                         \\ \bottomrule
% B1-P1                          & B1-P2  & \multicolumn{1}{c|}{B1-P3}  & B2-P1 & B2-P2 & \multicolumn{1}{c|}{B2-P3} & B3-P1         & B4-P1         & B5-P1        & ...        \\
% B1-P1                          & B1-P2  & \multicolumn{1}{c|}{B1-P3}  & B2-P1 & B2-P2 & \multicolumn{1}{c|}{B2-P3} & B3-P2         & B4-P2         & B5-P2        & ...        \\
% B1-P1                          & B1-P2  & \multicolumn{1}{c|}{B1-P3}  & B2-P1 & B2-P2 & \multicolumn{1}{c|}{B2-P3} & B3-P3         & B4-P3         & B5-P3        & ...        \\
% $\vdots$                             & $\vdots$        & \multicolumn{1}{c|}{$\vdots$}        & $\vdots$       & \vdots       & \multicolumn{1}{c|}{$\vdots$}       & $\vdots$               &  $\vdots$              & $\vdots$              &  $\ddots$          \\ \bottomrule
% \end{tabular}
% \end{table*}

==> tabs/videos_info_1.tex <==
\begin{table}[]
	\footnotesize
	\centering
	\caption{Touch Indicator Detection Accuracy}
	\label{tab:videos_info_1}
	\begin{tabular}{|l|c|c|c|c|}
		\toprule
		\textbf{App}&\textbf{Avg. Length}&\textbf{Avg. S2R}\\
		\midrule
		APOD	&	\approx21	&	\approx5\\
		GROW	&	\approx22	&	\approx7\\
		TIME	&	\approx25	&	\approx10\\
		TOK	&	\approx22	&	\approx7\\
		DROID	&	\approx24	&	\approx6\\
		GNU	&	\approx39	&	\approx13\\
		\bottomrule
	\end{tabular}
	%\vspace{-0.3cm}
\end{table}

